Accretion disks with a large scale magnetic field around black holes, and magnetic jet collimation

We discuss the problem of the formation of a large-scale magnetic field in the accretion disks around black holes, taking into account the nonuniform vertical structure of the disk. The high electrical conductivity of the outer layers of the disk prevents the outward diffusion of the magnetic field. This implies a stationary state with a strong magnetic field in the inner parts of the accretion disk close to the black hole, and zero radial velocity at the surface of the disk. Magnetic jet collimation is considered, when the jet radius is hold due to magneto-torsional oscillations. The range of parameters is found where jet radius is oscillating, regularly or chaotically, within restricted values.

==> standard-defs.tex <==
\newcommand{\dummy}{}
% Preprint formatting
\newenvironment{inlinefigure}{ 
\def\@captype{figure} 
\noindent\begin{minipage}{0.999\linewidth}\begin{center}} 
{\end{center}\end{minipage}\smallskip} 
%
% general
\newcommand{\etal}{{\em et al.}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\tnm}{\tablenotemark}
\newcommand{\aam}{\altaffilmark}
% misc astronomy
\newcommand{\HI}{H\mbox{\sc\small ~I~}}
\newcommand{\HII}{H\mbox{\sc\small ~II~}}
\newcommand{\kms}{km s$^{-1}$}
% VLBI 
\newcommand{\mas}{milliarcsecond}
\newcommand{\thetavec}{\mbox{\boldmath $\theta$}}
% ISS analysis
\newcommand{\dtd}{\Delta t_{\rm d}}
\newcommand{\dnud}{\Delta\nu_{\rm d}}
\newcommand{\Viss}{V_{\rm ISS}}
\newcommand{\Vissu}{V_{\rm ISS,5/3,u}} 
\newcommand{\Aissu}{A_{\rm ISS, 5/3, u}}
\newcommand{\Wc}{W_{\rm C}}
\newcommand{\Wdpm}{W_{\rm D,PM}}
\newcommand{\Vpperp}{{V_p}_{\perp}}
\newcommand{\Cnsqr}{C_n^2}
\newcommand{\Cnsqrtc}{C_{n,{\rm TC93}}^{2}}
\newcommand{\Cnsqrs}{C_{n,s}^2}
\newcommand{\dSM}{\Delta\mbox{SM}}
\newcommand{\dDM}{\Delta\mbox{DM}}
\newcommand{\Ds}{\Delta s}
\newcommand{\tc}{\mbox{\small TC93}}

